Tracking Objects with 3D Representation from Videos

Data association is a knotty problem for 2D Multiple Object Tracking due to the object occlusion. However, in 3D space, data association is not so hard. Only with a 3D Kalman Filter, the online object tracker can associate the detections from LiDAR. In this paper, we rethink the data association in 2D MOT and utilize the 3D object representation to separate each object in the feature space. Unlike the existing depth-based MOT methods, the 3D object representation can be jointly learned with the object association module. Besides, the object's 3D representation is learned from the video and supervised by the 2D tracking labels without additional manual annotations from LiDAR or pretrained depth estimator. With 3D object representation learning from Pseudo 3D object labels in monocular videos, we propose a new 2D MOT paradigm, called P3DTrack. Extensive experiments show the effectiveness of our method. We achieve new state-of-the-art performance on the large-scale Waymo Open Dataset.

==> sections/intro.tex <==
\section{Introduction}


Multiple Object Tracking (MOT) is the core component of the perception system for many applications, such as autonomous driving and video surveillance. Accuraltely associating the same object in each frame and keeping the trajectory as long as possible are crucial for MOT. In the deep learning era, metric learning helps the network to learn better object affinity between frames~\cite{wojke2017simple,braso2020learning,He_2021_CVPR}. Besides, end-to-end MOT~\cite{zhou2020tracking,zhang2021fairmot}, which learns object detection and object similarity jointly in the same neural network, becomes a new trend. Multiple Object Tracking can be divided into 2D MOT and 3D MOT according to the input modality. Generally speaking, 2D MOT aims to track the object from a video clip and 3D MOT tracks the object from LiDAR or multi-modality (e.g., LiDAR and images) in the 3D space.\par


% It connects the upstream task (object detection, instance segmentation) and downstream task (trajectory prediction and planning). Associating the same object in each frame keeping the trajectory as long as the object can be observed and are crucial for MOT.
% If data association cannot be solved, the wrong association, such as tracklet early termination and ID switch between two tracklets, can cause the wrong observation for the downstream task. The decision mistakes will be dangerous for the passengers and the passers-by.

% In the deep learning era, metric learning helps the network to learn better object affinity between frames~\cite{}. And end-to-end MOT~\cite{} begins to become the new trend, which combines object detection learning and similarity learning in the same neural network. 
In 2D MOT, due to the object occlusion on the image, the object association across the frame is one of the most challenging problems, even with the help of the appearance models and the motion models. When many objects are partially visible, like the scene of traffic jams and crowded shopping malls, the wrong association is very common. However, in 3D MOT, many works reveal that only with a simple motion model, the association is no more a hard problem. Recently, ImmortalTracker~\cite{wang2021immortal} points out that using 3D Kalman Filter to model the motion of the 3D bounding boxes from LiDAR, the wrong association is only \emph{once} in the whole Waymo Open Dataset (WOD) dataset. \emph{Why there is a huge gap in the association difficulty between 2D and 3D MOT?} In this paper, we want to rethink the data association problem in 2D MOT and bridge the gap between 2D and 3D MOT.\par
\begin{figure*}
          \centering
           \includegraphics[width=\linewidth]{figures/fig1.pdf}
             \caption{}
             \label{fig1}
\end{figure*}  
So, we try to lift the object into 3D space and represent the object not only with the 2D appearance but also with the implicit 3D feature. Recent works~\cite{hu2019joint, Khurana_2021_ICCV, dendorfer2022quo} utilize the off-the-shelf depth model to lift each pixel into the camera frame and try to separate the different objects. However, only applying the scene-level depth estimation is also hard to represent the object. It's hard to estimate the depth accurately, especially on the object boundary. However, the object boundary is the key to separating the objects, which means the depth estimation and object representation are coupled in these methods.\par
Different from these works, we learn 3D representation on the object level. Inspired by the structure-from-motion~\cite{schoenberger2016sfm}, the scene can be reconstructed from the camera motion. Distinct from the pretrained or LiDAR-supervised depth estimation, we utilize geometric constraints from the video. With the 2D object bounding boxes, the reconstructed point clouds can be naturally divided into different clusters. So, we learn the implicit 3D representation in the global frame instead of the depth in each frame from these 3D point clusters. With the global implicit 3D object representation, we propose a new end-to-end 2D MOT paradigm, called \methodname{}.\par
\textcolor{red}{TODO: description of I3DTrack.}\par
In summary, our work has the following contributions:
\begin{itemize}
\item We propose a new 2D MOT paradigm, learning the implicit 3D object representation and 2D object detection jointly.
\item We design the implicit 3D object representation learning module, only supervised by the 2D tracking labels without LiDAR or pretrained depth estimator.
\item The extensive experiments on the large-scale Waymo Open Dataset show that we achieve new state-of-the-art performance on 2D MOT.
\end{itemize}
